Clinical Utility Gains from Incorporating Comorbidity and Geographic Location Information into Risk Estimation Equations for Atherosclerotic Cardiovascular Disease

Objective: There are several efforts to re-learn the 2013 ACC/AHA pooled cohort equations (PCE) for patients with specific comorbidities and geographic locations. With over 363 customized risk models in the literature, we aim to evaluate such revised models to determine if the performance improvements translate to gains in clinical utility. Methods: We re-train a baseline PCE using the ACC/AHA PCE variables and revise it to incorporate subject-level geographic location and comorbidity information. We apply fixed effects, random effects, and extreme gradient boosting models to handle the correlation and heterogeneity induced by locations. Models are trained using 2,464,522 claims records from Optum Clinformatics Data Mart and validated in the hold-out set (N=1,056,224). We evaluate models' performance overall and across subgroups defined by the presence or absence of chronic kidney disease (CKD) or rheumatoid arthritis (RA) and geographic locations. We evaluate models' expected net benefit using decision curve analysis and models' statistical properties using several discrimination and calibration metrics. Results: The baseline PCE is miscalibrated overall, in patients with CKD or RA, and locations with small populations. Our revised models improved both the overall (GND P-value=0.41) and subgroup calibration but only enhanced net benefit in the underrepresented subgroups. The gains are larger in the subgroups with comorbidities and heterogeneous across geographic locations. Conclusions: Revising the PCE with comorbidity and location information significantly enhanced models' calibration; however, such improvements do not necessarily translate to clinical gains. Thus, we recommend future works to quantify the consequences from using risk calculators to guide clinical decisions.

==> Clinical Utility of Risk Estimation Equations for Atherosclerotic Cardiovascular Disease/Tables/Table1.tex <==
\begin{table}
\centering
\caption{Summary of Baseline Characteristics in Optum ZIP and STARR data. Continuous variables are summarized as mean and standard deviation and categorical variables are summarized as count and percentage. The total sample size (including ineligible patients) of  are 16,792,476 and 262,161, respectively.}
\label{t:summary}
\begin{tabular}{lcc}
\hline
Variable & Optum ZIP (N = 3,520,746) & STARR (N = 28,896) \\ \hline
Age (years) &	53.5 (9.9) &	55.9 (9.4)\\
Female     &	2,116,013 (57.4\%)&	16,316 (56.5\%)\\
Current Smoker	& 328,486 (8.9\%)	& 24,449 (84.6\%)\\
High-density Lipoproten         &	55.8 (17.4)&	58.1 (16.4)\\
Total Cholesterol &	197.0 (37.1) &	195.0 (34.2)\\
Antihypertensives  & 1,081,759 (29.3\%) &	4,193 (14.5\%)\\
Diabetes &	499,243 (13.5\%)&	1,894 (6.6\%)\\
Hypertension &	1,439,459 (39.0\%)&	7,194 (24.7\%)\\
Chronic Kidney Disease      	& 	109,116 (3.0\%) &	640 (2.2\%)\\
Rheumatoid Arthritis 	        &	64,641 (1.8\%)&	232 (0.8\%)\\
Systolic Blood Pressure         &	--  &	126.4 (16.6)\\
\multicolumn{3}{l}{Race and Ethnicity}	\\
\,\,\,Black or African American &	-- &	2,168 (7.5\%)\\
\,\,\,White   & -- &	26,728 (92.5\%)\\
\hline
\end{tabular}
\end{table}

==> Clinical Utility of Risk Estimation Equations for Atherosclerotic Cardiovascular Disease/Tables/Table2.tex <==
\begin{table}[ht]
\centering
\caption{Overall model performance for estimating the five-year ASCVD risk. \emph{Calib} and \emph{NB} denote calibration and net benefits, respectively. Compared to the baseline PCE, revised risk models improved the calibration performance significantly but only slightly increased the net benefits.}
\label{t:overall_org_pce}
\begin{tabular}{llcccc}
  \hline
Evaluation & Subtype & Baseline PCE & Fixed Effects & Random Effects & XGB \\ 
  \hline 
  C-index & -- & 0.69 (0.69, 0.70) & \textbf{0.70 (0.70, 0.71)} & 0.69 (0.69, 0.70) & 0.69 (0.69, 0.70) \\ \hline
   O/E    & -- & \textbf{1.01 (1.00, 1.02)} & \textbf{1.01 (1.00, 1.02)} & 1.05 (1.04, 1.06) & \textbf{1.01 (1.00, 1.02)} \\ 
  GND & -- & 150.6 ($<$ 0.001) & 113.7 (0.17) & 183.0 ($<$ 0.001) & \textbf{102.5 (0.41)} \\
  \multirow{2}{*}{Calib} & Intercept & \textbf{0.11 (0.10, 0.11)} & 0.12 (0.12, 0.12) & 0.11 (0.11, 0.11) & 0.11 (0.11, 0.11) \\ 
   & Slope & \textbf{1.28 (1.27, 1.29)} & 1.31 (1.30, 1.32) & 1.28 (1.27, 1.29) & 1.29 (1.28, 1.30) \\ \hline
   \multirow{2}{*}{NB} & 2.5\%  & \textbf{0.0736} & 0.0733 & 0.0734 & \textbf{0.0736} \\
                    & 3.75\% & 0.0623 & \textbf{0.0627} & 0.0624 & 0.0625 \\ 
                    & 10\% & 0.0291 & \textbf{0.0295} & 0.0290 & 0.0294 \\  \hline
\end{tabular}
\end{table}

==> Clinical Utility of Risk Estimation Equations for Atherosclerotic Cardiovascular Disease/Tables/Table3.tex <==
\begin{table}
\caption{Model performance across comorbidity subgroups. The baseline PCE is miscalibrated in all subgroups. \emph{Subtype} shows the risk thresholds for the net benefit metric. Revised models significantly improved subgroup model calibration and yielded nontrivially higher net benefits in the positive CKD and RA groups under the threshold of 10\%.}
\label{t:sub_org_pce}
\centering
\resizebox{\textwidth}{!}{\begin{NiceTabular}{lllcccc}[colortbl-like]
  \hline
Evaluation & Subgroup & Subtype & Baseline PCE & Fixed Effects & Random Effects & XGB \\
  \hline
  \multirow{4}{*}{C-index} & CKD = 0 & -- & 0.69 (0.68, 0.70) & \textbf{0.70 (0.69, 0.71)} & 0.69 (0.68, 0.70) & 0.69 (0.69, 0.70) \\ 
                           & \cellcolor{Gray}CKD = 1 & \cellcolor{Gray}-- & \cellcolor{Gray}0.61 (0.58, 0.64) & \cellcolor{Gray}\textbf{0.62 (0.59, 0.65)} & \cellcolor{Gray}0.61 (0.58, 0.64) & \cellcolor{Gray}\textbf{0.62 (0.59, 0.65)} \\ 
                           & RA = 0 & --  & 0.69 (0.69, 0.70) & \textbf{0.70 (0.70, 0.71)} & 0.69 (0.69, 0.70) & 0.70 (0.69, 0.70) \\ 
                           & \cellcolor{Gray}RA = 1 & \cellcolor{Gray}--  & \cellcolor{Gray}0.64 (0.60, 0.68) & \cellcolor{Gray}\textbf{0.65 (0.62, 0.69)} & \cellcolor{Gray}0.64 (0.60, 0.68) & \cellcolor{Gray}0.65 (0.61, 0.68) \\ \hline
  \multirow{4}{*}{O/E} & CKD = 0 & -- & \textbf{1.00 (0.99, 1.01)} & 1.01 (1.00, 1.02) & 1.06 (1.05, 1.07) & 1.01 (1.00, 1.02) \\ 
                       & \cellcolor{Gray}CKD = 1 & \cellcolor{Gray}-- & \cellcolor{Gray}1.09 (1.05, 1.13) & \cellcolor{Gray}\textbf{1.00 (0.96, 1.04)} & \cellcolor{Gray}\textbf{1.00 (0.96, 1.04)} & \cellcolor{Gray}\textbf{1.00 (0.96, 1.04)} \\ 
                       & RA = 0  & -- & \textbf{1.00 (0.99, 1.01)} & 1.01 (1.00, 1.02) & 1.05 (1.04, 1.06) & 1.01 (1.00, 1.02) \\ 
                       & \cellcolor{Gray}RA = 1  & \cellcolor{Gray}-- & \cellcolor{Gray}1.29 (1.22, 1.36) & \cellcolor{Gray}\textbf{1.00 (0.94, 1.05)} & \cellcolor{Gray}1.07 (1.01, 1.13) & \cellcolor{Gray}\textbf{1.00 (0.95, 1.06)} \\ \hline
  \multirow{4}{*}{GND} & CKD = 0 & -- & 161.1 ($<$ 0.001) & 106.5 (\textbf{0.28}) & 161.2 ($<$ 0.001) & 111.3 (0.19) \\ 
                       & \cellcolor{Gray}CKD = 1 & \cellcolor{Gray}-- & \cellcolor{Gray}53.8 (0.005) & \cellcolor{Gray}55.0 (0.004) & \cellcolor{Gray}60.2 ($<$ 0.001) & \cellcolor{Gray}31.2 (\textbf{0.40}) \\ 
                       & RA = 0 & --  & 136.5 (0.009) & 98.7 (\textbf{0.52}) & 164.1 ($<$ 0.001) & 118.5 (0.10) \\ 
                       & \cellcolor{Gray}RA = 1 & \cellcolor{Gray}--  & \cellcolor{Gray}77.3 ($<$ 0.0001) & \cellcolor{Gray}38.6 (0.040) & \cellcolor{Gray}51.0 (0.002) & \cellcolor{Gray}43.6 (0.012) \\ \hline
  \multirow{8}{*}{Calib} & \multirow{2}{*}{CKD = 0} & Intercept & \textbf{0.10 (0.10, 0.11)} & 0.12 (0.11, 0.12) & 0.11 (0.10, 0.11) & 0.11 (0.10, 0.11) \\ 

                         && Slope     & \textbf{1.28 (1.27, 1.29)} & 1.31 (1.30, 1.32) & \textbf{1.28 (1.27, 1.29)} & \textbf{1.28 (1.27, 1.29)} \\ 
                         & \multirow{2}{*}{\centering \cellcolor{Gray}CKD = 1} & \cellcolor{Gray}Intercept & \cellcolor{Gray}0.11 (0.10, 0.12) &\cellcolor{Gray} 0.11 (0.10, 0.13) &\cellcolor{Gray} 0.11 (0.10, 0.12) & \cellcolor{Gray}\textbf{0.10 (0.09, 0.12)} \\ 
                         &  \cellcolor{Gray}  & \cellcolor{Gray}Slope     & \cellcolor{Gray}1.10 (1.07, 1.14) & \cellcolor{Gray}1.12 (1.08, 1.16) & \cellcolor{Gray}1.10 (1.07, 1.14) & \cellcolor{Gray}\textbf{1.10 (1.06, 1.13)} \\ 
                         & \multirow{2}{*}{RA = 0}  & Intercept & \textbf{0.11 (0.10, 0.11)} & 0.12 (0.11, 0.12) & 0.11 (0.11, 0.11) & 0.11 (0.11, 0.11) \\ 
                         &                          & Slope     & \textbf{1.28 (1.27, 1.29)} & 1.31 (1.30, 1.32) & \textbf{1.28 (1.27, 1.29)} & 1.29 (1.28, 1.30) \\ 
                         & \cellcolor{Gray}\multirow{2}{*}{RA = 1}  & \cellcolor{Gray}Intercept & \cellcolor{Gray}0.11 (0.10, 0.13) & \cellcolor{Gray}0.12 (0.10, 0.14) & \cellcolor{Gray}0.11 (0.10, 0.13) & \cellcolor{Gray}\textbf{0.11 (0.09, 0.13)} \\ 
                         &   \cellcolor{Gray}                       & \cellcolor{Gray}Slope     & \cellcolor{Gray}\textbf{1.14 (1.09, 1.20)} & \cellcolor{Gray}1.18 (1.13, 1.23) & \cellcolor{Gray}\textbf{1.14 (1.09, 1.20)} & \cellcolor{Gray}\textbf{1.14 (1.09, 1.20)} \\ \hline
   \multirow{8}{*}{NB} & \multirow{3}{*}{CKD = 0}& 2.5\% & 0.0709 & 0.0706 & 0.0708 & \textbf{0.0710} \\ 
                      &                          & 3.75\% & 0.0596 & \textbf{0.0600} & 0.0597 & 0.0598 \\
                      &                          & 10\% & 0.0270 & \textbf{0.0274} & 0.0269 & 0.0272 \\ 
                      & \multirow{3}{*}{\cellcolor{Gray}CKD = 1} & \cellcolor{Gray}2.5\% &\cellcolor{Gray} 0.1711 & \cellcolor{Gray}0.1709 & \cellcolor{Gray}\textbf{0.1712} & \cellcolor{Gray}\textbf{0.1712} \\ 
                      &         \cellcolor{Gray}                 & \cellcolor{Gray}3.75\% & \cellcolor{Gray}0.1600 & \cellcolor{Gray}0.1598 & \cellcolor{Gray}0.1601 & \cellcolor{Gray}\textbf{0.1603} \\ 
                      &         \cellcolor{Gray}                 & \cellcolor{Gray}10\% & \cellcolor{Gray}0.1044 & \cellcolor{Gray}0.1045 & \cellcolor{Gray}0.1045 & \cellcolor{Gray}\textbf{0.1071} \\
                      & \multirow{3}{*}{RA = 0}  & 2.5\% & 0.0725 & 0.0722 & 0.0724 & \textbf{0.0726} \\ 
                      &                          & 3.75\% & 0.0613 & \textbf{0.0617} & 0.0614 & 0.0614 \\
                      &                          & 10\% & 0.0285 & \textbf{0.0289} & 0.0284 & 0.0288 \\
                      & \cellcolor{Gray}\multirow{3}{*}{RA = 1}  & \cellcolor{Gray}2.5\% & \cellcolor{Gray}0.1278 & \cellcolor{Gray}0.1278 & \cellcolor{Gray}0.1278 & \cellcolor{Gray}0.1278 \\
                      & \cellcolor{Gray}                         & \cellcolor{Gray}3.75\% & \cellcolor{Gray}0.1143 & \cellcolor{Gray}0.1153 & \cellcolor{Gray}0.1153 & \cellcolor{Gray}\textbf{0.1162} \\  
                      & \cellcolor{Gray}                         & \cellcolor{Gray}10\% & \cellcolor{Gray}0.0620 & \cellcolor{Gray}\textbf{0.0659} & \cellcolor{Gray}0.0632 &\cellcolor{Gray} 0.0643 \\  \hline
\end{NiceTabular}}
\end{table}

==> Clinical Utility of Risk Estimation Equations for Atherosclerotic Cardiovascular Disease/Tables/TableS1.tex <==
\begin{table}[ht]
\centering
\caption{Overall performance of the 2013 ACC/AHA PCE and the re-trained baseline PCE in STARR. The surrogate baseline PCE resulted in similar discrimination performance as the ACC/AHA PCE but worse calibration and net benefits.}
\label{t:overall_starr}
\begin{tabular}{lcccc}
  \hline
                   & 2013 ACC/AHA PCE &  Re-trained Baseline PCE \\\hline
 C-index & 0.69 (0.66, 0.72) & 0.70 (0.67, 0.73) \\\hline
 GND & 83 ($<$0.0001) & 3827 ($<$0.0001) \\\hline
\multicolumn{3}{l}{Net benefit}\\
\,\,\,2.5\% & 0.0227 & 0.0181 \\ 
\,\,\,3.75\% & 0.0168 & 0.0058 \\ 
\,\,\,10\% & 0.0022 & -0.0208 \\ 
\hline
\end{tabular}
\end{table}



==> Clinical Utility of Risk Estimation Equations for Atherosclerotic Cardiovascular Disease/Tables/TableS2.tex <==
\begin{table}[ht]
\centering
\caption{Discrimination of the baseline PCE evaluated by two different concordance metrics. Applying the IPCW C-statistic where censoring is modeled as a function of covariates \citep{gerds2013estimating} yielded very similar results as the Harrell's C-statistic that assumes noninformative censoring \citep{pencina2004overall}.}
\label{t:cindex_comp}
\begin{tabular}{lcc}
  \hline
         & Harrell's C-statistic    & IPCW C-statistic \\\hline
 Overall & 0.69 (0.69, 0.70) & 0.69 \\\hline
 CKD=1   & 0.61 (0.58, 0.64) & 0.62 \\\hline
 CKD=0   & 0.69 (0.68, 0.70) & 0.69 \\
\hline
\end{tabular}
\end{table}


==> Clinical Utility of Risk Estimation Equations for Atherosclerotic Cardiovascular Disease/Tables/TableS3.tex <==
\begin{table}[ht]
\centering
\caption{Concept and concept codes used to extract the Optum and STARR cohorts.}
\label{t:concept_code}
\begin{tabular}{ll}
  \hline
 Concept                  & Code \\\hline
 Cardiovascular disease (ICD-9)&  410*, 411*, 413*, 414*, 430*, 431*, \\
 & 432*, 433*, 434*, 436*, 427.31, 428*\\
 Coronary heart disease (ICD-9)& 411*, 413*, 414*\\
 Myocardial infarction (ICD-9)& 410*\\
 Stroke (ICD-9)& 430*, 431*, 432*, 433* (exclude 433.*0), \\
 & 434* (exclude 434.*0), 436*\\
 Hypertension (ICD-9) & 401*, 402*, 403*, 404*, 405*\\
 Type 1 diabetes (SNOMED) & 46635009, 444073006, 420868002\\
 Type 2 diabetes (SNOMED) & 74627003, 268519009, 73211009\\
 Chronic kidney disease (SNOMED) & 42399005, 28689008, 36171008, 709044004, 197661001,\\
 & 38481006, 52254009, 52845002, 127013003, 36184004 \\
 & (exclude 50581000, 733839001, 102455002, 43629001, \\
 & 198949009, 200118004, 707742001, 14669001, 609452007\\
 Rheumatoid arthritis (SNOMED) & 69896004\\
 Statin (ATC) & C10AA0[1-8]\\
 Systolic blood pressure (LONIC) & 76534-7, 8479-8, 8480-6\\
 High-density lipoprotein (LONIC) & 12772-0, 54372-8, 2085-9, 27340-9, 14646-4, \\	
& 12771-2, 53135-0, 18263-4, 50840-8, 49130-8\\
 Total cholesterol (LONIC)& 12183-0, 14647-2, 2093-3\\\hline
\end{tabular}
\end{table}


==> Clinical Utility of Risk Estimation Equations for Atherosclerotic Cardiovascular Disease/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
